Persona Knowledge-Aligned Prompt Tuning Method for Online Debate

Debate is the process of exchanging viewpoints or convincing others on a particular issue. Recent research has provided empirical evidence that the persuasiveness of an argument is determined not only by language usage but also by communicator characteristics. Researchers have paid much attention to aspects of languages, such as linguistic features and discourse structures, but combining argument persuasiveness and impact with the social personae of the audience has not been explored due to the difficulty and complexity. We have observed the impressive simulation and personification capability of ChatGPT, indicating a giant pre-trained language model may function as an individual to provide personae and exert unique influences based on diverse background knowledge. Therefore, we propose a persona knowledge-aligned framework for argument quality assessment tasks from the audience side. This is the first work that leverages the emergence of ChatGPT and injects such audience personae knowledge into smaller language models via prompt tuning. The performance of our pipeline demonstrates significant and consistent improvement compared to competitive architectures.

==> emnlp2023-latex/sections/abstract.tex <==
\begin{abstract}
Debate is the process of exchanging viewpoints or convincing others on a particular issue. Recent research has provided empirical evidence that the persuasiveness of an argument is determined not only by language usage but also by communicator characteristics. Researchers have paid much attention to aspects of languages, such as linguistic features and discourse structures, but combining argument persuasiveness and impact with the social personae of the audience has not been explored due to the difficulty and complexity. We have observed the impressive simulation and personification capability of ChatGPT, indicating a giant pre-trained language model may function as an individual to provide personae and exert unique influences based on diverse background knowledge. Therefore, we propose a persona knowledge-aligned framework for argument quality assessment tasks from the audience side. This is the first work that leverages the emergence of ChatGPT and injects such audience personae knowledge into smaller language models via prompt tuning. The performance of our pipeline demonstrates significant and consistent improvement compared to competitive architectures.
\end{abstract}

==> emnlp2023-latex/sections/conclusion.tex <==
\section{Conclusion}
This paper introduces a persona knowledge-aligned prompt tuning method for tackling online debate argument tasks by utilizing audience persona knowledge. Our proposed framework elicits this persona knowledge from a large language model (i.e., ChatGPT).  
The performance of our model exhibits significant and consistent improvement against competitive baselines. We hope our comprehensive discussions will provide valuable insights for communities in computational argumentation. 



==> emnlp2023-latex/sections/ethics_statement.tex <==
\section*{Ethics Statement}
In this work, we conformed to recognized privacy practices and rigorously followed the data usage policy. We declare that all authors of this paper acknowledge the \emph{ACM Code of Ethics} and honor the code of conduct. 
This paper presents a method to utilize generated audience persona knowledge from ChatGPT to provide more signals to enhance the model performance on two online debate tasks. All generated persona knowledge reflects the selection and reporting biases~\cite{gordon2013reporting} of ChatGPT, which could sometimes be stereotypical and do not represent the views of the authors. However, we took the following steps to mitigate this effect. Firstly, we design an explicit prompt to instruct the ChatGPT to generate optimistic attributes about personas, which has been shown in prior work to reduce the toxicity of outputs~\cite{DBLP:journals/tacl/SchickUS21}. Second, we performed the human evaluations on the 1,000 sampled persona knowledge generated from ChatGPT and did not observe any harmful and toxic language resulting from the ChatGPT fine-tuned with the RLHF approach~\cite{DBLP:conf/nips/ChristianoLBMLA17}, which prevents ChatGPT from generating harmful and toxic language without deliberate attacks~\cite{DBLP:conf/nips/ChristianoLBMLA17}. Nevertheless, it is essential to acknowledge that none of these safeguards are perfect. We cannot guarantee that all generated persona knowledge does not contain any undesired or harmful content, and expert annotators may possess varying perspectives on what constitutes toxic content~\cite{DBLP:conf/naacl/SapSVZCS22}.

==> emnlp2023-latex/sections/experiments.tex <==
\section{Experimental Setting}
\subsection{Task Datasets}
To validate the effectiveness of persona knowledge in debate tasks, we conducted experiments on two tasks: argument impact classification in the \textit{Kialo} dataset \cite{DBLP:conf/emnlp/DurmusLC19} and argument persuasion prediction in the \textit{DDO} dataset~\cite{DBLP:conf/acl/DurmusC19, DBLP:conf/emnlp/LiDC20}. The Kialo dataset collected various topics and categorized the user votes into three impact classes (\textit{Not Impactful, Medium Impact,} and \textit{Impactful}) based on agreement and the number of valid votes to reduce noise. The dataset statistics are presented in Table~\ref{table:stat_label} in Appendix~\ref{sec:appendix_data_statistics}. The \textit{DDO} dataset is used for the argument persuasion prediction task. The task involves predicting the winner who presented more convincing arguments in a debate. Each debate consists of multiple rounds, with each round featuring an utterance from the PRO side and one from the CON side. More details can be found in Appendix~\ref{sec:appendix_data_statistics}.

\subsection{PresonaPrompt Implementation Details}
We employ Flan-T5~\cite{DBLP:journals/corr/abs-2210-11416}, which uses instructions to tune the T5 model~\cite{DBLP:journals/jmlr/RaffelSRLNMZLL20}, as the PLM backbone in \textbf{PersonaPrompt}. For fair comparison with various baselines, we used Flan-T5-base as the primary model.
In general, the overall configuration follows the setup in \citet{DBLP:conf/emnlp/LesterAC21}, and more configuration details can be found in Appendix~\ref{sec:appendix_discoPrompt_implementation_details}.
Following previous works~\cite{DBLP:conf/emnlp/DurmusLC19, DBLP:conf/acl/LiuOSJ20, DBLP:conf/emnlp/LiDC20}, we report the Macro-F1 score for the argument impact classification task and ablation study, while accuracy is reported for the argument persuasion prediction task. All experiments are conducted using 2 $\times$ NVIDIA V100 (32GB) GPUs.
% We employ the Flan-T5 model~\cite{DBLP:journals/corr/abs-2210-11416} as the PLM backbone in \textbf{PersonaPrompt}. 
% The overall configuration generally follows the setting in \citet{DBLP:conf/emnlp/LesterAC21} and sets the learnable prompt length as 20. The batch size and maximum input sequence are 4 and 512, respectively. The maximum generated sequence length of the encoder is 10. For these two tasks, the training was implemented using cross-entropy loss with 30,000 training steps, which selects the model that yields the best performance on the validation set. We adopt an Adafactor~\cite{DBLP:conf/icml/ShazeerS18} optimizer and perform grid search with learning rates \{3e-6, 4e-6, 5e-6\} in Kialo dataset and grid search with learning rates \{3e-7, 4e-7, 5e-7\} in DDO dataset. Our model is conducted on two 32GB NVIDIA V100 GPUs. The running time for Flan-T5-base is around 8 hours, while Flan-T5-large is about 22 hours. 

\subsection{Baselines}
This paper mainly adopts two categories of competitive baselines for the \textit{Kialo} dataset and the \textit{DDO} dataset. The first category consists of the previous state-of-the-art baselines, such as LR~\cite{DBLP:conf/emnlp/DurmusLC19}, SVM~\cite{DBLP:conf/acl/DurmusC19}, BiLSTM~\cite{DBLP:conf/acl/LiuOSJ20}, HAN-BiLSTM~\cite{DBLP:conf/acl/LiuOSJ20}, BERT~\cite{DBLP:conf/emnlp/DurmusLC19}, and DisCOC~\cite{DBLP:conf/acl/LiuOSJ20}.
The other category involves the fine-tuned Flan-T5 models to illustrate the performance gain of prompt tuning. Additionally, we include general Prefix-Tuning~\cite{DBLP:conf/acl/LiL20} as well as Prompt-Tuning~\cite{DBLP:conf/emnlp/LesterAC21}. 
The details of the baselines and their implementation are listed in Appendix~\ref{sec:appendix_experiments}.



\begin{table*}[!t]
    \centering
    \small
    \scalebox{0.75}{\begin{tabular}{l|c c c}
    \toprule
    \multicolumn{1}{c|}{\textbf{Model}} &  \multicolumn{1}{c}{\textbf{Precision}} &  \multicolumn{1}{c}{\textbf{Recall}} &  \multicolumn{1}{c}{\textbf{Macro F1}} \\ 
    \midrule
    \textsc{Majority} & 19.43 & 33.33 & 24.55 \\
    \textsc{SVM}~\cite{DBLP:conf/emnlp/DurmusLC19} & 65.67 & 38.58 & 35.42 \\
    % FastText & 51.18 $\pm$ 0.80 & 46.09 $\pm$ 0.64 & 47.06 $\pm$ 0.70 \\
    \textsc{BiLSTM}~\cite{DBLP:conf/acl/LiuOSJ20} & 46.94 $\pm$ 1.08 & 46.64 $\pm$ 0.71 & 46.51 $\pm$ 1.11 \\
    % \hline
    \textsc{HAN-BiLSTM}~\cite{DBLP:conf/acl/LiuOSJ20} & 51.93 $\pm$ 1.37 & 49.08 $\pm$ 1.52 & 50.00 $\pm$ 1.49 \\
    \textsc{BERT~\cite{DBLP:conf/emnlp/DurmusLC19}} & 57.19 $\pm$ 0.92 & 55.77 $\pm$ 1.05 & 55.98 $\pm$ 0.70 \\
    \textsc{DisCOC}~\cite{DBLP:conf/acl/LiuOSJ20} & 57.90 $\pm$ 0.70 & 59.41 $\pm$ 1.41 & 58.36 $\pm$ 0.52 \\
    
    \hline
    \textsc{Fine-Tuning (Flan-T5-base)}~\cite{DBLP:journals/jmlr/RaffelSRLNMZLL20} & 58.48 $\pm$ 1.04 & 59.57 $\pm$ 0.54 & 58.45 $\pm$ 0.69\\
    \textsc{Fine-Tuning (Flan-T5-base) (Knowledge)}~\cite{DBLP:journals/jmlr/RaffelSRLNMZLL20}  & 60.37 $\pm$ 1.73 & 60.58 $\pm$ 0.21 & 60.10 $\pm$ 1.25\\
    \textsc{Fine-Tuning (Flan-T5-large)}~\cite{DBLP:journals/jmlr/RaffelSRLNMZLL20} & 58.95 $\pm$ 0.81 & 63.42 $\pm$ 0.52 & 60.23 $\pm$ 0.23 \\
    \textsc{Fine-Tuning (Flan-T5-large) (Knowledge)}~\cite{DBLP:journals/jmlr/RaffelSRLNMZLL20} & 62.63 $\pm$ 1.04 & 64.56 $\pm$ 0.56 & 63.31 $\pm$ 0.68\\ 

    \textsc{Prompt-Tuning (Flan-T5-base)}~\cite{DBLP:conf/emnlp/LesterAC21} & 61.05 $\pm$ 1.58 & 57.80 $\pm$ 0.76 & 58.61 $\pm$ 0.84\\
    \textsc{Prompt-Tuning (Flan-T5-base) (Knowledge)}~\cite{DBLP:conf/emnlp/LesterAC21} & 60.52 $\pm$ 0.32 & 59.78 $\pm$ 0.62 & 59.58 $\pm$ 0.69\\
    \textsc{Prompt-Tuning (Flan-T5-large)}~\cite{DBLP:conf/emnlp/LesterAC21} & 63.48 $\pm$ 1.33 & 63.13 $\pm$ 0.78 & 63.10 $\pm$ 0.77\\  

    \textsc{Prompt-Tuning (Flan-T5-large)(Knowledge)}~\cite{DBLP:conf/emnlp/LesterAC21} & 65.18 $\pm$ 1.03 &  \underline{65.12} $\pm$ 0.75 & 65.20 $\pm$ 0.46\\
    \textsc{Prefix-Tuning (Flan-T5-base)}~\cite{DBLP:conf/acl/LiL20} & 61.95 $\pm$ 2.03 & 57.69 $\pm$ 1.44 & 58.35 $\pm$ 1.24\\
    \textsc{Prefix-Tuning (Flan-T5-base) (Knowledge)}~\cite{DBLP:conf/acl/LiL20} & 61.85 $\pm$ 1.43 & 60.96 $\pm$ 0.17 & 60.13 $\pm$ 0.22\\
    \textsc{Prefix-Tuning (Flan-T5-large)}~\cite{DBLP:conf/acl/LiL20} & 65.01 $\pm$ 0.95 & 62.10 $\pm$ 1.25 & 62.87 $\pm$ 1.01\\

    \textsc{Prefix-Tuning (Flan-T5-large) (Knowledge)}~\cite{DBLP:conf/acl/LiL20} & \underline{65.43} $\pm$ 1.53 & 65.09 $\pm$ 0.64 & \underline{65.25} $\pm$ 0.71\\
    \hline
    
    \textsc{PersonaPrompt (Flan-T5-base)} & 59.19 $\pm$ 0.57 & 60.20 $\pm$ 0.67 & 59.29 $\pm$ 0.67\\
    \textsc{PersonaPrompt (Flan-T5-base) (Knowledge)} & 64.35 $\pm$ 0.63 & 62.11 $\pm$ 0.36 & 62.81 $\pm$ 0.31\\
    \textsc{PersonaPrompt (Flan-T5-large)} & 65.40 $\pm$ 0.54 &64.26 $\pm$ 1.08 &  64.35 $\pm$ 0.51\\ 

    \textsc{PersonaPrompt (Flan-T5-large) (Knowledge)} & \bf{68.48} $\pm$ 1.24 & \bf{67.16} $\pm$ 0.58 &  \bf{67.77} $\pm$ 0.54 \\  
    \bottomrule
    \end{tabular}}
    \vspace{-0.3cm}
    \caption{The mean and standard deviation of the performance of different models on argument impact classification task (i.e., \textit{Kialo} dataset). \textsc{Knowledge} indicates incorporating with the generated audience persona knowledge. The upper portions are the previous SOTA methods, and the middle portions are the implemented baselines.}
    \label{table:arg_impact_main}
    \vspace{-0.6cm}
\end{table*}

\begin{table}[!t]
    \centering
    \small
    % \vspace{-0.5cm}
    \setlength\tabcolsep{2pt}
    \scalebox{0.75}{\begin{tabular}{l|c}
    \toprule
    \multicolumn{1}{c|}{\textbf{Model}} &  \multicolumn{1}{c}{\textbf{Accuracy}} \\ 
    \midrule
    \textsc{Majority} & 62.62 \\
    \textsc{Linguistic+User LR}& 67.41 \\
    \textsc{Arg-Struct LR} & 69.52 \\
    \textsc{Linguistic+Arg-Struct LR} & 70.48 \\
    \textsc{Linguistic+User+Arg-Struct LR} & 70.44 \\
    \hline
    \textsc{BERT} & 64.71 $\pm$ 0.73\\
    \textsc{BERt(Knowledge)} & 66.09 $\pm$ 1.27\\
    \textsc{DisCOC} & 64.48 $\pm$1.03\\
    \textsc{DisCOC(Knowledge)} & 67.01 $\pm$ 1.17\\
    \hline
    \textsc{Fine-Tuning (Flan-T5-base)} & 70.15 $\pm$ 0.58\\
    \textsc{Fine-Tuning (Flan-T5-base)(Knowledge)}  & 72.87 $\pm$ 0.12\\
    \textsc{Fine-Tuning (Flan-T5-large)} & 71.75 $\pm$ 0.59\\
    \textsc{Fine-Tuning (Flan-T5-large)(Knowledge)}  & 73.25 $\pm$ 0.41\\
    \hline
    \textsc{Prefix-Tuning (Flan-T5-base)} & 68.62 $\pm$ 0.77\\
    \textsc{Prefix-Tuning (Flan-T5-base)(Knowledge)} & 71.26 $\pm$ 0.49\\
    \textsc{Prefix-Tuning (Flan-T5-large)} & 70.69 $\pm$ 0.79\\ 
    \textsc{Prefix-Tuning (Flan-T5-large)(Knowledge)} & 73.41 $\pm$ 0.58\\
    \hline
    \textsc{Prompt-Tuning (Flan-T5-base)} & 68.01 $\pm$ 1.38\\
    \textsc{Prompt-Tuning (Flan-T5-base)(Knowledge)} & 71.61 $\pm$ 0.63\\
    \textsc{Prompt-Tuning (Flan-T5-large)} & 71.26  $\pm$ 1.22\\  
    \textsc{Prompt-Tuning (Flan-T5-large)(Knowledge)} & \underline{73.64} $\pm$ 0.49\\
    \hline
    \textsc{PersonaPrompt (Flan-T5-base)} & 71.08 $\pm$ 0.70\\
    \textsc{PersonaPrompt (Flan-T5-base)(Knowledge)} & 73.45 $\pm$ 0.34\\
    \textsc{PersonaPrompt (Flan-T5-large)} & 72.56 $\pm$ 1.06\\
    \textsc{PersonaPrompt (Flan-T5-large)(Knowledge)} &  \bf{75.86} $\pm$ 0.43\\
    \bottomrule
    \end{tabular}}
    \vspace{-0.3 cm}
    \caption{The performance of the models on the argument persuasion prediction task (i.e., \textit{DDO} dataset), where the upper portions of baselines are Logistic Regression (LR) models with the linguistic feature, user information, and argument structure~\cite{DBLP:conf/emnlp/LiDC20}.}
    % ${\diamond}$ \textbf{ : as in Liu et al.}\cite{DBLP:conf/acl/LiuOSJ20}.
    \label{table:DDO_main}
    \vspace{-0.6cm}
\end{table}


\section{Experimental Result}
\subsection{Main Results}
Table~\ref{table:arg_impact_main} and Table~\ref{table:DDO_main} summarize the main results of the two online debate tasks, which include the argument impact classification task and argument persuasion task, from which we derive the following conclusions.
\textbf{First}, our method significantly outperforms all baselines in both tasks and achieves state-of-the-art (SOTA) performance in the argument impact classification task. Specifically, our method (Flan-T5-large and Flan-T5-base) outperforms previous SOTA \textsc{DisCOC}~\cite{DBLP:conf/acl/LiuOSJ20} with at least 9.41\% and 4.45\% F1 scores in the argument impact classification task.
\textbf{Second}, our model gains a considerable improvement of 7.54\% F1 score and 4.11\% accuracy over the fine-tuning of the Flan-T5-large (without persona knowledge) model in the \textit{Kialo} and \textit{DDO} datasets. It demonstrates that our method effectively utilizes the audience persona knowledge, perceives this specific knowledge on the correlation of knowledge and the data argument and context, and finally enhances the ability of Flan-T5 to undertake this challenging task.
\textbf{Third}, all models fine-tuned or prompt-tuned with the knowledge exhibit improvement over original tuning. In particular, PersonPrompt (knowledge) with the Flan-T5-base version obtained a 3.52\% F1 score gain in performance over original tuning without persona knowledge. It illustrates the effectiveness of the generated persona knowledge on the online debate quality assessment tasks.
% \xin{More baselines and results can be found in Append~\ref{sec:appendix_baseline_models}.}







\begin{table}[!t]
% \begin{minipage}{0.43\textwidth}
% \vspace{-0.2cm}
\centering
\scalebox{0.6}{\begin{tabular}{l|l|l|l}
\toprule
\multicolumn{1}{c|}{\textbf{Model}} &  \multicolumn{1}{c|}{\textbf{Precision}} &  \multicolumn{1}{c|}{\textbf{Recall}} &  \multicolumn{1}{c}{\textbf{F1}} \\ 
\hline
\textsc{Majority} & 19.43 & 33.33 & 24.55 \\
\textsc{ChatGPT (baseline)} & 40.20 & 33.84 & 34.26 \\
\textsc{ChatGPT (w knowledge)} & 39.04 & 37.18 & 36.60 \\
\textsc{GPT-4 (baseline)} & 50.00 & 44.84 & 39.52 \\
\textsc{GPT-4 (w knowledge)} & 56.14 & 44.19 & 41.60 \\
\hline
\textsc{ChatGPT (A.)} & 47.30 & 33.98 & 26.46  \\ 
\textsc{ChatGPT (A. \& K.)} & 40.55 & 39.03 & 28.44 \\
\textsc{ChatGPT (C. \& A.)} & 41.20 & 34.84 & 35.26 \\
\textsc{ChatGPT (C. \& A.\& K.)} & 39.04 & 37.18 & 36.60  \\
\hline
\end{tabular}}
\vspace{-0.3cm}
\caption{The performance of ChatGPT (\textit{gpt-3.5-turbo-0125}) and GPT-4 (\textit{gpt-4-turbo-2024-04-09}) on the argument impact task. The bottom part is the ChatGPT model performance for the ablation study on the data input. \textsc{C.}, \textsc{A.}, and \textsc{K.} present context, argument, and persona knowledge, respectively.
}
\label{tab:ChatGPT_Performance}
% \end{minipage}
\vspace{-0.6cm}
\end{table}

\subsection{Knowledge Adaptation on Large Language Models}
With the remarkable ability demonstrated by LLMs across a diverse array of tasks~\cite{DBLP:journals/corr/abs-2303-12712,DBLP:journals/corr/abs-2302-04023,DBLP:conf/eacl/ChanCWJFLS24}, we are intrigued about the capability of large language models on zero-shot online debate tasks. We employ the prompting template in \citet{DBLP:conf/iclr/RobinsonW23} to formulate the task as a multiple choice question answering problem as a baseline and append with the audience persona knowledge to compare with this baseline. 
The prompting template is displayed in Figure~\ref{fig:ChatGPT_prompt_tempalte} in Appendix~\ref{sec:Implementation_Details_of_LLMs}.
We test the performance of ChatGPT (\textit{gpt-3.5-turbo-0125})~\cite{openai2022chatgpt} and GPT-4 (\textit{gpt-4-turbo-2024-04-09})~\cite{DBLP:journals/corr/abs-2303-08774} on the argument impact classification task, and the performance is presented in Table~\ref{tab:ChatGPT_Performance}. Although all designed templates perform better than the majority baseline, their overall performance remains suboptimal compared to supervised learning. This result reveals that argument impact classification is still tricky for ChatGPT and cannot be solved easily at the current state, resulting from the argument quality assessment task requiring more ability than only comprehending the semantic meaning of the arguments presented in a debate. As shown in Table~\ref{tab:ChatGPT_Performance}, the context plays a significant role in ChatGPT's zero-shot performance in this task. Moreover, we observed a slight improvement in performance after concatenating knowledge with the pre-designed templates and demonstrated that persona knowledge is also effective for ChatGPT.
% \begin{figure}[!t]
%     % \vspace{-0.5 cm}
%     \centering
%     \includegraphics[width=\linewidth]{sections/Figures/ChatGPT_Template.pdf}
%     \vspace{-0.8 cm}
%     \caption{Prompting template for large language models. The upper part is the baseline template refer to \citet{DBLP:conf/iclr/RobinsonW23}, and the bottom part is the prompt template with the persona knowledge.
%     }
%     \label{fig:ChatGPT_prompt_tempalte}
%     \vspace{-0.6 cm}
% \end{figure}

\subsection{Ablation Study on PersonaPrompt}
To better investigate the factors of PersonaPrompt, we design numerous ablations on the various aspects of PersonaPrompt on argument impact classification task.
% Table~\ref{table:arg_impact_ablationstudy} reports the performance of the ablation study for our model in the argument impact classification task.
\begin{table}[!t]
    \centering
    \small
    \setlength\tabcolsep{1.5pt}
    % \vspace{-0.2cm}
    \scalebox{0.75}{\begin{tabular}{l|c|c|c}
    \toprule
    \multicolumn{1}{c|}{\textbf{Model}} &  \multicolumn{1}{c}{\textbf{Precision}} &  \multicolumn{1}{c}{\textbf{Recall}} &  \multicolumn{1}{c}{\textbf{F1}} \\ 
    \midrule
    % \textsc{PersonaPrompt (A.)} & 56.94 & 56.08 & 56.28\\
    \textsc{PersonaPrompt (A.)} & 56.94 & 56.08 & 56.28\\
    \textsc{PersonaPrompt (A. \& C.)} & 59.19 & 60.20 & 59.29\\
    \textsc{PersonaPrompt (A. \& K.)} & 60.52 & 60.15 & 60.23\\
    \textsc{PersonaPrompt (A. \& C. \& K.)} & \textbf{64.35} & \textbf{62.11} & \textbf{62.81}\\
    
    \hline
    
    \textsc{BERT (A.)} &  53.24 & 50.93 & 51.53 \\
    \textsc{BERT (A. \& C.)} & 57.19 & 55.77 & 55.98 \\
    \textsc{BERT (A. \& K.)} & 53.52 & 54.94 & 53.59 \\
    \textsc{BERT (A. \& C. \& K.)} & 56.76 & 58.55  & 57.25 \\
    \textsc{DisCOC (A. \& C.)} & 57.90 & 59.41 & 58.36 \\
    \textsc{DisCOC (A. \& C. \& K.)} & 57.83 & 59.94 & 58.69 \\

    \textsc{Flan-T5 (A.)} & 49.26 & 54.99 & 50.44\\
    \textsc{Flan-T5 (A. \& C.)} & 58.48 & 59.57 & 58.45 \\
    \textsc{Flan-T5 (A. \& K.)} & 54.39 & 58.16 & 55.62\\
    \textsc{Flan-T5 (A. \& C. \& K.)} & 60.37 & 60.58 & 60.10\\
    \bottomrule
    \end{tabular}
    }
    \vspace{-0.3cm}
    \caption{The ablation study on the argument impact classification task, where  \textsc{C.}, \textsc{A.}, and \textsc{K.} stands for context, argument, and persona knowledge, respectively. Note that DisCOC must require the context due to its recurrent mechanism. Flan-T5 indicates the Fine-Tuning (Flan-T5-base) model.
    % Cont. means only use 1 context length
    }
    \label{table:arg_impact_ablationstudy}
    \vspace{-0.5cm}
\end{table}

\paragraph{Can Knowledge Replace Context}
The context has demonstrated significant influences on the model performance in prior works~\cite{DBLP:conf/emnlp/DurmusLC19, DBLP:conf/acl/LiuOSJ20}, so we wonder whether persona knowledge can be used to replace the context.
As the experimental results reported in Table~\ref{table:arg_impact_ablationstudy}, we draw the following conclusions:
(1) Context significantly contributes to the performance of various models;
(2) Persona knowledge can be utilized to replace certain information or signals from the context, aiding the model in determining the class label and emphasizing the importance of knowledge;
(3) Incorporating persona knowledge alongside the context consistently improves model performance.



\begin{figure}[!t]
    % \vspace{-0.2cm}
    \centering
    \includegraphics[width=0.8\linewidth]{sections/Figures/Crop_Context_Length.pdf}
    \vspace{-0.4cm}
    \caption{F1 scores of different models on varying the context numbers. The results of HAN, Flat, and Interval-RoBERTa are referenced from~\citet{DBLP:conf/acl/LiuOSJ20}. The distinguishing factor among these models lies in the form of context modeling.}\label{fig:path_len}
    \vspace{-0.4cm}
\end{figure}

\paragraph{Influence of the Context Length}
Different debate claims have different context lengths in the Kailo dataset. 
Figure~\ref{fig:path_len} shows F1 scores of models with different context lengths. 
Only \textsc{PresonaPrompt (Knowledge)} and \textsc{DisCOC} benefit from longer discourse contexts, while other models get stuck in performance fluctuation. \textsc{PresonaPrompt (Knowledge)} and \textsc{DisCOC} have consistent performance gains; instead, other models cannot learn long-distance structures better. With the persona knowledge, the PLMs can receive extra signals to perceive the semantics meanings of longer context.

\paragraph{Prompt Engineering} Furthermore, we conduct the prompt template searching and the parameter sensitivity on the continuous prompt length that we describe in Appendix~\ref{sec: Appendix_ablation_study_PersonaPrompt}.









\subsection{In-depth Exploring on Persona Knowledge}



\paragraph{Are All Persona Dimensions Helpful}
Experiments are conducted on all four dimensions of persona knowledge to verify the effectiveness of each dimension. Based on the result presented in Table~\ref{table:arg_impact_dimension_ablationstudy}, it can be concluded that the persona argument is the most essential dimension of the persona that contributes to the model performance. For instance, as demonstrated in Figure~\ref{fig:DataInstance_Introduction}, the computer science professor persona instantiates low-level concepts such as memory management, hardware interactions, and performance optimization in the argument, thereby providing extensive information to strengthen their viewpoint on the debate topic for pre-trained language models to undertake this task. Moreover, other dimensions also provide additional signals to help the pre-trained language models determine the impact and persuasiveness of the argument.

\begin{table}[!t]
    \centering
    \small
    % \vspace{0.5cm}
    \scalebox{0.65}{
    \begin{tabular}{l|c c c}
    \toprule
    \multicolumn{1}{c|}{\textbf{Model}} &  \multicolumn{1}{c}{\textbf{Precision}} &  \multicolumn{1}{c}{\textbf{Recall}} &  \multicolumn{1}{c}{\textbf{F1}} \\ 
    \midrule
    \textsc{PersonaPrompt (w/o knowledge)}  & 59.19 $\pm$ 0.57 & 60.20 $\pm$ 0.67 & 59.29 $\pm$ 0.67\\
    \textsc{PersonaPrompt (w Knowledge)} & \bf{64.35} $\pm$ 0.63 & \bf{62.11} $\pm$ 0.36 & \bf{62.81} $\pm$ 0.31\\
    \hline
    \textsc{PersonaPrompt (R \& S)} & 61.06 $\pm$ 0.86 & 61.38 $\pm$ 1.26 & 60.63 $\pm$ 1.34\\
    \textsc{PersonaPrompt (R \& A)} & 61.54 $\pm$ 1.03 & 61.38 $\pm$ 1.20 & 61.26 $\pm$ 1.61\\
    \textsc{PersonaPrompt (R \& C)} & 61.57 $\pm$ 0.77 & 60.70 $\pm$ 0.62 & 60.85 $\pm$ 0.29\\
    \textsc{PersonaPrompt (R \& I)} & 62.29 $\pm$ 0.76 & 60.65 $\pm$ 0.78 & 60.79 $\pm$ 1.31\\ 
    \textsc{PersonaPrompt (R \& A \& S)} & 62.10 $\pm$ 0.88 & 62.98 $\pm$ 0.81 & 62.09 $\pm$ 1.25\\
    \textsc{PersonaPrompt (R \& A \& C)} & 61.07 $\pm$ 0.89 & 63.10 $\pm$ 0.85 & 61.67 $\pm$ 0.84\\
    \textsc{PersonaPrompt (R \& A \& I)} & 62.77 $\pm$ 1.22 & 62.26 $\pm$ 0.59 & 62.29 $\pm$ 0.12\\
    \textsc{PersonaPrompt (R \& S \& A \& C)} & 62.74  $\pm$ 1.12 & 62.51 $\pm$ 0.82 & 62.44 $\pm$ 0.48\\ 
    \textsc{PersonaPrompt (R \& S \& A \& I)} & 63.97 $\pm$ 0.83 & 61.94 $\pm$ 0.68 & 62.73 $\pm$ 1.13\\  
    \hline
    
    \textsc{PersonaPrompt (1 Persona)} & 61.18 $\pm$ 1.04 & 58.84 $\pm$ 0.79 & 59.58 $\pm$ 1.17\\
    \textsc{PersonaPrompt (2 Personae)} & 61.03 $\pm$ 1.30 & 60.49 $\pm$ 0.64 & 60.60 $\pm$ 1.15\\
    \textsc{PersonaPrompt (3 Personae)} & 61.62 $\pm$ 1.12 & 60.66 $\pm$ 0.92 & 61.05 $\pm$ 0.56\\
    \textsc{PersonaPrompt (4 Personae)} & 62.50 $\pm$ 0.74 & 63.27 $\pm$ 1.06 & 61.98 $\pm$ 0.93\\
    \textsc{PersonaPrompt (5 Personae)} & 63.98 $\pm$ 1.13 & 61.94 $\pm$ 1.01 & 62.67 $\pm$ 1.10\\
    \hline 
    \textsc{PersonaPrompt (Con)} & 60.33 $\pm$ 0.88 & 61.99 $\pm$ 0.89 & 61.05 $\pm$ 0.44 \\
    \textsc{PersonaPrompt (Pro)} & 61.07 $\pm$ 0.90 & 60.73 $\pm$ 0.94 & 60.79 $\pm$ 0.62 \\
    \textsc{PersonaPrompt (Neutral)} & 63.15 $\pm$ 0.87 & 62.05 $\pm$ 0.96 & 61.95 $\pm$ 0.75\\
    \bottomrule
    \end{tabular}
    }
    \vspace{-0.2cm}
    \caption{The ablation study on persona knowledge on the argument impact classification task. \textsc{R}, \textsc{S}, \textsc{A}, \textsc{C}, and \textsc{I} represent role, stance, argument, character, and intent.
    }
    \label{table:arg_impact_dimension_ablationstudy}
    \vspace{-0.6 cm}
\end{table}

\paragraph{Influence of Persona Number}
To obtain a more profound comprehension of the effect of persona number on the model performance, a series of experiments are designed with varying quantities of persona, with results illustrated in Table~\ref{table:arg_impact_dimension_ablationstudy}. Generally, it is observed that an increase in the number of personae leads to a corresponding increase in the model performance, with noteworthy enhancement in the 3.09\% F1 score observed when five personae were employed as opposed to 1 persona. However, the optimal PersonaPrompt (persona knowledge) equipped with more than five personas does not observe significant benefits, and it may result from the limited maximum sequence length of model input. 




\paragraph{Are Stance Group Helpful}
To probe a deeper understanding of the stance group of persona (i.e., \textsc{Pro, Con}, and \textsc{Neutral}) contributed to the performance, we divided the persona into three distinct groups and performed experiments with the same quantity of persona in each group. To ensure a fair comparison, we opt for all the persona knowledge within these three groups that possess similar token lengths.
Table~\ref{table:arg_impact_dimension_ablationstudy} reveals an intriguing finding that the \textsc{neutral} group outperforms the other groups. 
Specifically, the P-values for the \textsc{Neutral} group are 0.0286 and 0.0493 (paired student’s t-test, p < 0.05) against the \textsc{PRO} and \textsc{CON} groups. One rationale may be the \textsc{Neutral} group persona knowledge encoding more information or signal on both sides instead of just a single side and their stances, as illustrated by the example depicted in Figure~\ref{fig:DataInstance_Introduction}.







\begin{table}[!t]
\small
\centering
% \vspace{-0.4cm}
% \begin{minipage}{0.54\textwidth}
\scalebox{0.75}{\begin{tabular}{l|l|l|l}
\toprule
\multicolumn{1}{c|}{\textbf{Model}} &  \multicolumn{1}{c|}{\textbf{Precision}} &  \multicolumn{1}{c|}{\textbf{Recall}} &  \multicolumn{1}{c}{\textbf{F1}} \\ 
\hline
\textsc{w/o knowledge}& 59.19 $\pm$ 0.57 & 60.20 $\pm$ 0.67 & 59.29 $\pm$ 0.67\\
\textsc{ConceptNet (Triple)}& 60.20 $\pm$ 0.80 & 59.59 $\pm$ 1.13 & 59.46 $\pm$ 0.35 \\
\textsc{ConceptNet (Language)} & 60.09 $\pm$ 0.82 & 61.08 $\pm$ 0.78 & 59.89 $\pm$ 0.75 \\
\textsc{Background knowledge} & 61.21 $\pm$ 1.22 & 60.59 $\pm$ 0.98 & 60.09 $\pm$ 1.10 \\
\textsc{Persona knowledge} & 64.35 $\pm$ 0.63 & 62.11 $\pm$ 0.36 & 62.81 $\pm$ 0.31\\
\hline
\end{tabular}}
\vspace{-0.4cm}
\caption{The performance of PersonaPrompt (Flan-T5-base) with various knowledge resources on the argument impact task. \textsc{Triple} and \textsc{Language} correspond to the ConceptNet knowledge representation forms in triple and natural language, respectively.
}
% \vspace{-0.4cm}
\label{tab:KnowledegSource_Performance}
% \end{minipage}
\vspace{-0.5cm}
\end{table}

\begin{figure*}[!t]
    % \vspace{-0.3cm}
    \centering
    \includegraphics[width=0.7\linewidth]{emnlp2023-latex/sections/Figures/Attention Visualization.pdf}
    \vspace{-0.3cm}
    \caption{Attention visualization for \textsc{Fine-Tuning (FLAN-T5-base) (Knowledge)} on the example shown in Figure~\ref{fig:DataInstance_Introduction}.
    }\label{fig:Attention_Visualization}
    \vspace{-0.7cm}
\end{figure*}

\subsection{Knowledge Type Comparison}
We undertake a comparison of the generated persona knowledge with the commonsense knowledge from ConceptNet and background knowledge generated from ChatGPT to assess the exact contribution of persona knowledge and the effectiveness of different knowledge on this argument impact classification task. ConceptNet~\cite{DBLP:conf/aaai/SpeerCH17} is a widely used and traditional knowledge graph consisting of 42 relation types. By following the \textsc{KagNet} method~\cite{DBLP:conf/emnlp/LinCCR19}, we ground the ConceptNet knowledge on the argument and context of the Kailo dataset. The case example of retrieved commonsense knowledge can be found in Figure~\ref{fig:ConceptNet_Knowledge} and Figure~\ref{fig:ConceptNet_Knowledge_1} in Appendix~\ref{sec:More_case_ConceptNet}. Furthermore, we crafted a prompt template, "Please list all relevant background knowledge regarding the argument and context," to generate the background knowledge from ChatGPT. After receiving all retrieved knowledge, we substitute the persona knowledge with the commonsense or background knowledge in our designed input template shown in Figure~\ref{fig:DiscoursePrompt_Architecture}. There are two representations of commonsense knowledge from ConceptNet, which are the triple and natural language representing forms. 
The outcome is reported in Table~\ref{tab:KnowledegSource_Performance} and indicates that the ConceptNet knowledge does not make a significant improvement on this task. The reason behind this result may be the retrieval of much noisy and contextually irrelevant knowledge from the traditional knowledge graph that damages the model performance. This problem remains a challenging research question~\cite{DBLP:conf/emnlp/LinCCR19}, while our generated persona knowledge from ChatGPT obtained a high human evaluation score on the relevance aspect. Moreover, the persona knowledge model obtains a significant performance gap against the background knowledge, and it evidences the efficacy of multi-dimensional persona knowledge.  





\subsection{Attention Visualization}
To further examine the impact of persona knowledge on this argument impact classification task, we display how the model (i.e., \textsc{Fine-Tuning (Flan-T5-base) (Knowledge)}) assigns weight to different input elements by using an attention visualization tool~\cite{alammar2020explaining}, and the resulting visualization is shown in Figure~\ref{fig:Attention_Visualization}. Interestingly, the Self-taught Programmer contributes the highest weights among all persona roles and even surpasses the weight contributed by the context. A neutral persona and their argument seem to provide more information and weights to assist PLMs in determining the class label, which is consistent with previous findings. More cases of attention visualization can be found in Appendix~\ref{sec:More_case_Attention_Visualization}.

% \begin{figure}[!t]
%     % \vspace{-0.3cm}
%     \centering
%     \includegraphics[width=\linewidth]{sections/Figures/Attention Visualization.pdf}
%     \vspace{-0.3cm}
%     \caption{Attention visualization for fine-tuning (Flan-T5-base) (Knowledge) on the example shown in Figure~\ref{fig:DataInstance_Introduction}.
%     }\label{fig:Attention_Visualization}
%     \vspace{-0.5cm}
% \end{figure}




==> emnlp2023-latex/sections/introduction.tex <==
\section{Introduction}
In the field of Natural Language Processing (NLP) and Computational Argumentation, there is a burgeoning research interest in studies to develop computational methods that can automatically assess the qualitative characteristics of arguments.
The impact and persuasiveness of the argument are crucial and pivotal qualitative characteristics, and substantial research has been conducted to develop computing methodologies for identifying the impact and the persuasiveness of a natural language argument in public debate forums~\cite{DBLP:conf/emnlp/HabernalG16,DBLP:conf/acl/HabernalG16,DBLP:conf/www/TanNDL16,DBLP:conf/naacl/DurmusC18,DBLP:journals/tacl/SimpsonG18,DBLP:conf/emnlp/LiDC20}.
Nevertheless, estimating the impact or persuasiveness of an argument covering various debate topics requires more extensive knowledge
% (e.g., background knowledge and linguistics knowledge)
than merely comprehending the surface semantic meaning of an argument in online debate forums. In argumentation mining, \citet{DBLP:journals/tacl/LauscherWGG22} define the term \textbf{knowledge} as \textit{any kind of normative information that is considered to be relevant for solving a task at hand and that is not given as task input itself}.

\begin{figure}[t]
    % \vspace{-0.2 cm}
    \centering
    \includegraphics[width=\linewidth]{sections/Figures/DataInstance.pdf}
    \vspace{-0.7 cm}
    \caption{A data example from \textit{Kialo} and diverse audience personas generated by ChatGPT on this online debate topic. The \textit{Context} indicates the previous historical arguments from other users. The \textit{Argument} indicates the current argument or statement from the users.}
    \label{fig:DataInstance_Introduction}
    \vspace{-0.7 cm}
\end{figure}

Traditional works in argument assessment tasks have studied various aspects of knowledge~\cite{DBLP:journals/tacl/LauscherWGG22}. Among them, the impact and persuasiveness of arguments are inextricably linked not only to the linguistic attributes of the language~\cite{DBLP:conf/acl/WeiLL16} but also to the traits of the communicators, including the source (speakers)~\cite{DBLP:conf/www/DurmusC19}, 
the prior beliefs~\cite{DBLP:conf/naacl/DurmusC18},
argument structure~\cite{DBLP:conf/emnlp/LiDC20}, and the influence of discourse contexts~\cite{DBLP:conf/acl/LiuOSJ20}.
However, previous works have not well explored the analysis of the social personae of the audience in a computational manner, except by annotating human subjects on the speaker side~\cite{DBLP:conf/eacl/WalkerALW17}.
The recent computational studies for personae in Large Language Models (LLM) underscore the significance of personality information~\cite{jiang2023personallm,li2024personal}.
Furthermore, research in social psychology has identified the factors of argument persuasiveness, one of which is the \textbf{audience}~\cite{petty1986elaboration,johnson2013role, DBLP:journals/patterns/AlshomaryW21}, as a substantial amount of content is not expressed explicitly but resides in the mind of the audience~\cite{DBLP:journals/argcom/Moens18}, and the impact and persuasiveness of arguments are highly dependent on the audience.

Figure~\ref{fig:DataInstance_Introduction} illustrates various audience personae having various stances and interpretations on the same stated context and argument.
An individual's persona exerts significant influence on his/her own background knowledge (e.g., prior beliefs) and personality (e.g., roles' characters and intents)~\cite{DBLP:conf/naacl/DurmusC18}. Hence, diverse audience personas formulate different stances and arguments on a particular debate argument according to their characters and intentions.
Therefore, we adopt this focus since persona knowledge on the audience side plays a crucial role in forming stances and viewpoints about controversial topics and ultimately helps to determine the impact and persuasiveness of the argument.

Nevertheless, the challenge lies in the high level of difficulty and complexity associated with acquiring the audience's persona knowledge, and the manual collection imposes difficulty on the scalability of persona knowledge for various argument assessment tasks. 
Numerous works have successfully elicited knowledge from large language models instead of retrieving it on the knowledge graph~\cite{
DBLP:conf/emnlp/WangHQSWLG22}.
% DBLP:journals/corr/abs-2303-01903,DBLP:journals/corr/abs-2305-05252
ChatGPT~\cite{openai2022chatgpt} has demonstrated the ability to act in diverse roles given the instructions and applied for different tasks and areas~\cite{DBLP:journals/corr/abs-2305-14325,
DBLP:journals/corr/abs-2302-04023}, especially simulating an open world and the roles~\cite{DBLP:journals/corr/abs-2304-03442}.
% DBLP:journals/corr/abs-2305-14688, 
Hence, in this paper, we utilize ChatGPT imitation of various audience roles on each debate topic and argument, prompting persona knowledge through the tailored prompt to explore its influence on the argument assessment task. Furthermore, we proposed a persona knowledge-aligned framework for aligning the persona knowledge from LLM (i.e., ChatGPT) to a smaller language model (i.e., FLAN-T5) via prompt tuning to undertake the argument assessment task. The persona knowledge infuses into the tunable prefix prompt tokens without altering the pre-trained model representations.
Our contributions are summarized as follows:
{\begin{itemize}[leftmargin=*]
    \item To the best of our knowledge, this is the first work that explores and aligns audience persona knowledge into pre-trained language models via prompt tuning on the argument quality assessment task\footnote{The source code is available at~\url{https://github.com/HKUST-KnowComp/PersonaPrompt}}.
    \item We designed a framework to elicit human-validated audience persona knowledge from a large language model (i.e., ChatGPT) to help determine the impact and persuasiveness of the argument. 
    \item We conduct extensive experiments and thorough ablation studies to discuss the necessity and effectiveness of the various tailored dimensions of persona knowledge and the proposed method.
\end{itemize}}

==> emnlp2023-latex/sections/limitation.tex <==
\section*{Limitations}
\paragraph{Limited Persona Knowledge Dimensions}
First, the generated persona knowledge cannot be deemed comprehensive. Although we select four dimensions of personas based on the task, the generated persona knowledge cannot cover all dimensions of personas, nor all attributes of these dimensions.
Furthermore, since our generated persona knowledge only utilizes the context and argument from the dataset, the knowledge is task-specific on the online debate argument tasks, including the argument impact classification task and the argument persuasion prediction task.

\paragraph{Reporting biases Inherent in Pre-trained Language Model}
All elicited persona knowledge only comes from ChatGPT and its pre-training corpora. This constraint restricts the persona knowledge types, numbers, and role types for each debate topic owing to the reporting biases~\cite{gordon2013reporting} in the pre-trained language models (PLMs). This constraint consequently restricts the model capability in the online debate tasks.












% \paragraph{Limited language source}
% Finally, the primary language of all generated persona knowledge and dataset are English, making a solely English resource.

% \paragraph{Limited Utilized knowledge}
% Limited Information Utilized for Prompting knowledge}

% \paragraph{Limited Utilized Knowledge} The main limitation of our method is the limited utilized knowledge. Since our prompt tuning-based method tests on Implicit Discourse Relation Recognition (IDRR) task, the elicited knowledge only comes from the dataset of this task and the model pre-training corpora. This constraint restricts the capability owing to the reporting bias\cite{DBLP:conf/cikm/GordonD13} in the pre-training models (PLMs). Moreover, the relatively few training data of several second-level classes resulting from the highly skewed label distribution problem requires extensive knowledge to make the model understand data instances and the task. Although we impose the prior human knowledge against the IDRR task from the input template designing to the discourse connectives selection, the knowledge source still only comes from our prior knowledge and the elicited knowledge of PLMs. As a result, even our method obtains a valid score in all second-level classes except the \textit{Cont.Pragmatic Cause} displayed in Table~\ref{table:Label-wise F1}, some second-level senses, which are the same as previous studies, cannot receive a satisfactory performance (e.g.,~\textit{Comp.Concession} and~\textit{Expa.List}). The future work for this issue is to integrate more abundant knowledge and equip the model with more vital abilities. For example, grounding~\cite{DBLP:conf/emnlp/LinCCR19} on or retrieving the relevant nodes of the knowledge graph for each data instance provides more contextual information and enhances the capability of the model on this task.
 



% % 1. Limitation can show some case study for our model cannot perform well.
% % 7. case study for complicate case can run in T5-11B while connpromptPCP cannot solve 
% % or case study: have path vs havent path



==> emnlp2023-latex/sections/model.tex <==
\section{Persona Knowledge Aligned Prompt Framework}
\noindent \textbf{Problem Definition.}
Despite the differences in debate forms, the primary objective of debaters remains to persuade the audience effectively.
Therefore, our aim is to utilize machine learning methods to predict the winner of a debate based on the persuasiveness of their arguments.
This approach allows us to frame argument assessment tasks as classification problems giving an argument claim $\mathcal{A}$ and its corresponding context $\mathcal{C}$,
predict the label $\mathcal{Y} \in$ \{\textit{Con, Pro}\} in the debate form of DDO benchmark, while $\mathcal{Y} \in$ \{\textit{Impactful, Medium Impact, Not Impact}\} in Kialo debate forms. Therefore, this task is to find out the proper winner or plausible impact level based on the persuasiveness:

\scalebox{0.91}{\parbox{1.10\linewidth}{
\begin{align}
    y_{i}^{*}=\arg \max _{y_{i}^{j}} \text{Pr}\left(y_{i}=y_{i}^{j} \mid x_{i}^{j}\right),
\end{align}
}}
where $y_{i}^{*}$ is the most persuasive winner or most reasonable impact level, and $j$ indicates the $j$-th label among all labels.

\subsection{PersonaPrompt}
To predict the label $y_i$ for each instance $x_i = \{(c_i, a_i)\}$, we append the corresponding audience persona knowledge $p_i$ to each instance. Then, we leverage a human-tailored template $\mathcal{T}(\cdot)$ to convert the data instances and the persona knowledge to the prompt input $\tilde{x}_i = \mathcal{T}(p_i, x_i)$ and a verbalizer $\mathcal{V}(\cdot)$ to map a set of label words to class labels. Figure~\ref{fig:DiscoursePrompt_Architecture} illustrates the overall framework.

\noindent \textbf{Knowledge-Aligned Template}
The crafted template includes necessary discrete tokens and learnable continuous tokens.
As shown in Figure~\ref{fig:DiscoursePrompt_Architecture}, we utilize indicators to separate the ``context'' and ``argument'' and instruct the models to predict either the winner of the debate or the potential impact level of an argument.
In addition, we incorporate persona knowledge generated by ChatGPT as the ``background'' preceding the context, which aligns persona knowledge from a large language model to the small model to enhance the comprehension ability 
on the tasks, providing a broader and more comprehensive perspective on the debate process. 
We also appended 20 learnable continuous tokens at the beginning of the input template, allowing them to be updated through backpropagation.

\noindent \textbf{Verbalizer}
A traditional verbalizer $\mathcal{V}(\cdot)$ is a mapping function ($\mathcal{V}:  \mathcal{Y} \rightarrow \mathcal{Z} $) designed for bridging the set of answer token $\mathcal{Z}$ to the class label set $\mathcal{Y}$~\cite{DBLP:journals/corr/abs-2107-13586}. Normally, by using the prompt template and the function $\mathcal{V}(\cdot)$, the probability distribution over $\mathcal{Y}$ can be formalized as the probability distribution over $\mathcal{Z}$ at the masked position, i.e., $\text{Pr}(y_i | \tilde{x}_i) = \text{Pr}(\mathcal{V}(y_i)|\tilde{x}_i) = \text{Pr}(z_i| \tilde{x}_i)$.
To explicitly exhibit the contribution and effectiveness of persona knowledge in our model, we simplify the verbalizer function, which treats the original class label with lowercase as the label words (e.g., "Con" to "con").
Thus, we predict the label by choosing the higher probability answer token:\\
\scalebox{0.91}{\parbox{1.10\linewidth}{
\begin{align}
    y_{i}^{*}=\arg \max _{z_{i}^{j}} \text{Pr}\left(z_{i}=z_{i}^{j} \mid \tilde{x}_i^{j}\right).
\end{align}
}}
The final learning objective of PersonaPrompt is to maximize\\
\scalebox{0.91}{\parbox{1.10\linewidth}{
\begin{align}
    \mathcal{J} = \frac{1}{|\mathcal{D}|} \sum_{(x_i, y_i) \in \mathcal{D}} \log \text{Pr}\left(z_{i}=z_{i}^{j} \mid \tilde{x}_i^{j}\right).
\end{align}
}
}





==> emnlp2023-latex/sections/persona.tex <==
\section{Persona Knowledge}
\subsection{Persona Knowledge Generation}
\paragraph{Data Argument and Context} 
There are two forms of debate presented online. One is the arguments are typically structured as a series of rounds, with each round featuring an utterance from the PRO side and one from the CON side\footnote{To maintain consistency in methodology, we call a round with arguments from two debaters as one argument.} (e.g., \textit{DDO} dataset~\cite{DBLP:conf/acl/DurmusC19, DBLP:conf/emnlp/LiDC20}). 
In contrast, open debate platforms like \textit{Kialo}\footnote{\url{https://www.kialo.com/}} often adopt a more informal approach, allowing individuals to express their stances and argument claims to provide support or opposition to various topics or arguments, where the process can be organized as a debate tree.
We define the \textbf{argument claim} denoted as $\mathcal{A}$ to be the argumentative and persuasive text to express an idea for the audience and regard other relevant arguments in previous rounds or from other speakers as the \textbf{context} $\mathcal{C}$, $\mathcal{C}$ = $(\mathcal{C}^0, \mathcal{C}^1, \cdots, \mathcal{C}^{l})$ where $l$ is context length and $\mathcal{C}^{l}$ is the parent argument of $\mathcal{A}$. 


\begin{figure}[!t]
% \begin{minipage}{\textwidth}
    \vspace{-0.2cm}
    % \begin{minipage}[b]{0.5\textwidth}
    \centering
    \includegraphics[width=1.05\linewidth]{sections/Figures/ChatGPT_PromptTemplate3.pdf}
    \vspace{-0.7cm}
    \caption{The upper portion is a prompt template for eliciting the persona knowledge from ChatGPT, and the bottom portion is the randomized instruction generator.}
    \label{fig:ChatGPT_PromptTemplate}
    \vspace{-0.5cm}
    % \end{minipage}
\end{figure}

\paragraph{Dimensions of Persona Knowledge}
We notice that \citet{moore2019persona} proposed five common dimensions of persona: Public, Mediatized, Performative, Collective, and VARP (\textit{Values, Agency, Reputation, Prestige}) dimensions.
However, those dimensions are too general for debate arguments, which may not be specific and adaptable to broader debate topics. To construct efficient and task-specific representations of persona knowledge on the argument quality assessment task, we intuitively and meticulously design four potential dimensions for each persona knowledge instance as follows:

\noindent \textbf{Persona Stance} This dimension describes the stance of an audience persona (i.e., \textit{Con}, \textit{Pro}, or \textit{Neutral}) regarding the given argument and context. 
% For example, Figure~\ref{fig:DataInstance_Introduction} demonstrates the software engineer persona holds a \textit{Con} stance on the given data.

\noindent \textbf{Persona Argument} This dimension presents the audience persona argument that supports their stance, according to their own characters and intentions.

\noindent \textbf{Persona Characters} This dimension describes intrinsic character traits that a persona is likely to exhibit. 
% For instance, Figure~\ref{fig:DataInstance_Introduction} shows that the computer science professor is likely to possess traits such as knowledgeability and logical thinking.

\noindent \textbf{Persona Intent} This dimension outlines the external action or outcome that an audience persona intends to achieve or accomplish in the forthcoming period. Given that diverse audience personas take different stances and arguments on a specific debate argument according to their characters and intentions, this dimension is an integral part of persona knowledge in this work.
% For example, one possible intent of the computer science professor is \textit{to guide and educate students on the fundamentals of programming and provide insights into the benefits of learning C++}.

\paragraph{Persona Knowledge Generation}
To ensure the high quality and diversity of elicited multi-dimensional personae from ChatGPT\footnote{Disclaimer: All generated persona knowledge reflects the selection and reporting biases~\cite{gordon2013reporting} of ChatGPT, which could sometimes be stereotypical and do not represent the views of the authors.} and mitigate the issues of LLMs sensitive to instruction and few-shot examples~\cite{DBLP:conf/nips/PerezKC21}, we have customized the dynamic prompting template and introduced randomization in the prompts. This is achieved by \textbf{(I)} manually creating a collection of semantically similar instructions and randomly sampling from the instruction set each time, \textbf{(II)} creating an initial in-context examples pool, and dynamically sampling in-context examples for each input.
The initial in-context examples pool includes 100 manually refined persona knowledge for 10 well-chosen instances, which are crafted to cover as many relevant, critical, and diverse personas as possible.
The prompt template is displayed in Figure~\ref{fig:ChatGPT_PromptTemplate}, and an example of the persona knowledge generated by ChatGPT is presented in Figure~\ref{fig:DataInstance_Introduction}. For a given context $c_i \in \mathcal{C}$ and argument claim of $a_i \in \mathcal{A}$, by employing large language model $\mathcal{M}$, we sample persona knowledge $p_i \in \mathcal{P}$: 
\begin{align}
    p_i \sim \mathcal{M}(p_i \mid c_i, a_i)
\end{align}
where $i$ indicates $i$-th instance of the dataset $\mathcal{D}=\left\{\left(x_{i},y_{i}\right)\right\}_{i=1}^{|\mathcal{D}|}$ and $x_{i}=\left\{c_i, a_i\right\}$.
It is noteworthy that the persona knowledge generated by ChatGPT and GPT-4 exhibits significant similarity. We have opted for ChatGPT to generate all persona knowledge to optimize cost efficiency, and GPT-4 generated persona knowledge shown in Appendix~\ref{sec:More_case_GPT-4}.

\begin{figure}[!t]
    % \begin{minipage}[b]{0.5\textwidth}    
    \centering
    \vspace{-0.2cm}
    \includegraphics[width=0.85\linewidth]{sections/Figures/HumanEvaluationScore.pdf}
    \vspace{-0.15in}
    \caption{Human validation of five aspects of persona knowledge elicited from ChatGPT. The human evaluation score for the Harmfulness aspect is zero, indicating that no harmful or toxic language is found in the 1,000 sampled personae, which is omitted from the figure.}
    \label{fig:Human_Evaluation}
    \vspace{-0.5cm}
    % \end{minipage}
% \end{minipage}
\end{figure}

\begin{figure*}[!t]
% \vspace{-0.4cm}
% \small
\centering
\includegraphics[width=\textwidth]{sections/Figures/PresonaPrompt_Framework.pdf}
\vspace{-0.7cm}
\caption{
Overview of the PresonaPrompt framework.
}
\label{fig:DiscoursePrompt_Architecture}
\vspace{-0.5cm}
\end{figure*}


\subsection{Human Validation}
To assess the quality, effectiveness, and helpfulness of generated persona knowledge and to address potential hallucination issues in the generated content~\cite{DBLP:journals/corr/abs-2305-11747}, we conduct a human validation to complement the experimental results. 
We score each persona and the corresponding four dimensions of generated knowledge in the following intrinsic and extrinsic criteria:
(1) \textbf{Relevance} that determines whether the Roles, Argument, and Intent are relevant to the data argument and context;
(2) \textbf{Fluency} that assesses the fluency and understandability of the Roles, Argument, and Intent;
(3) \textbf{Consistency} that evaluates whether the Intent and Argument are consistent with Stance;
(4) \textbf{Plausibility} that gauges the reasonableness and plausibility of the Intent and Argument;
(5) \textbf{Usefulness} that measures whether the generation helps in determining the persuasiveness of the data argument;
(6) \textbf{Harmfulness} that estimates whether the generated knowledge includes harmful and toxic language or words.
% Intrinsic: Relevance, Fluency, Consistency, Plausibility
% Extrinsic: Usefulness

We randomly sample 1,000 persona roles from the 250 debates in the testing set, and five annotators are asked to evaluate every role in these dimensions, yielding a total of 30,000 ratings for all sampled knowledge (1,000 persona roles $\times$ 6 aspects $\times$ 5 annotators). We take the majority vote among five votes as the final result for each persona knowledge. The Inter-Annotator Agreement (IAA) score is 73.33\%, computed using pairwise agreement proportion, and Fleiss's Kappa~\cite{fleiss1971measuring} is 0.45. 
The average scores are in Figure~\ref{fig:Human_Evaluation}.
The relevance, fluency, consistency, and harmfulness aspects receive the higher agreement, while the plausibility and usefulness aspects obtain relatively lower agreement among annotators compared with other dimensions but also obtain 87\% and 79\% IAA scores. Notably, the harmfulness aspect in these 1,000 sample persona knowledge is zero, and a zero score means no harmful or toxic language is detected in the generation. It may be attributed to the ChatGPT fine-tuned with reinforcement learning from human feedback (RLHF) approach, which prevents ChatGPT from generating harmful language without deliberate attacks~\cite{DBLP:conf/nips/ChristianoLBMLA17}. 




==> emnlp2023-latex/sections/related_work.tex <==
\section{Related Work}
\subsection{Argument Persuasiveness Classification}
The study of computational argumentation has recently attracted more attention, which uses corpora collected from web argumentation sources like the CMV sub-forum of Reddit to assess the qualitative impact of arguments~\cite{DBLP:conf/www/TanNDL16}. There are many literature studies on the importance and efficacy of various aspects in determining the persuasiveness, including surface textual, social interaction, and argumentation-related features~\cite{DBLP:conf/acl/WeiLL16}, the characteristics of the source~\cite{DBLP:conf/www/DurmusC19} and audience~\cite{DBLP:conf/naacl/DurmusC18,DBLP:conf/um/Shmueli-Scheuer19}, the sequence ordering of argument~\cite{DBLP:conf/aaai/HideyM18}, and style feature aspects~\cite{DBLP:conf/acl/BaffWKS20}, were studied and investigated. Apart from the aforementioned features, 
% the importance of pragmatics and discourse context has been demonstrated but has not yet been fully investigated. Therefore, \citet{DBLP:conf/emnlp/DurmusLC19} construct a novel dataset by extracting the arguments and the impact votes from a debate platform kialo.com to launch a new study on the influence of discourse contexts on determining argument impact. 
\citet{DBLP:conf/emnlp/DurmusLC19} turned to the pragmatics and discourse context in the analysis of arguments.
They conducted experiments to demonstrate that the historical arguments are beneficial for the model performance to some extent. \citet{DBLP:conf/www/Zeng0HGLK20} and \citet{DBLP:conf/acl/LiuOSJ20} performed research on how the context and dynamic progress of argumentative conversation affect comparative persuasiveness in the debate process.
% Hence, in this work, we also consider the influence of contexts on the argument impact.


\subsection{Knowledge Elicitation from Pre-trained Language Models}
Considerable studies have demonstrated that Pre-trained Language Models (PLMs) have a substantial amount of knowledge implicitly stored that can be accessed via conditional generation~\cite{DBLP:conf/emnlp/PetroniRRLBWM19,DBLP:conf/emnlp/DavisonFR19, DBLP:journals/tacl/JiangXAN20}.
Additionally, the giant GPT-3~\cite{brown2020language} showed that manually designed prompts can tailor generations for diverse tasks in few-shot scenarios and achieve competitive results.
Accordingly, prompt tuning methods can use these language models to directly elicit knowledge to perform language understanding~\cite{DBLP:conf/emnlp/WangHQSWLG22,DBLP:journals/corr/abs-2305-05252} and commonsense reasoning~\cite{DBLP:conf/coling/YangLNTWL20,DBLP:conf/acl/ParanjapeMGHZ21,DBLP:conf/acl/0010LLWWBCH22}.
Recently, ChatGPT has demonstrated its ability to assume various roles and perform tasks in different domains based on given instructions~\cite{DBLP:journals/corr/abs-2305-14325, DBLP:journals/corr/abs-2305-14688, DBLP:journals/corr/abs-2305-02364, DBLP:conf/emnlp/JiangCCW23, DBLP:journals/corr/abs-2408-02559}, especially simulating an open world~\cite{DBLP:journals/corr/abs-2304-03442}.
Therefore, we employ ChatGPT to emulate the audience of diverse backgrounds in debates and utilize a prompt to inject persona knowledge into classifiers.
